Accurate Quality Elicitation in a Multi-Attribute Choice Setting

This paper studies how to accurately elicit quality for alternatives with multiple attributes. Two multiple price lists (MPLs) are considered: (i) m-MPL which asks subjects to compare an alternative to money, and (ii) p-MPL where subjects are endowed with money and asked whether they would like to buy an alternative or not. Theoretical results show that m-MPL requires fewer assumptions for accurate quality elicitation compared to p-MPL. Experimental evidence from a within-subject experiment using consumer products shows that switch points between the two MPLs are different, which suggests that quality measures are sensitive to the elicitation method.

==> Attribute/Tables/Regression_Entire_LinearTobit.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
%\begin{tabular}{l*{4}{D{.}{.}{-1}}}
\begin{tabular}{lcccc}
\toprule
                    & Linear            &Tobit             \\
                    & (1)               & (2)              \\
\midrule
Block               & $-0.918\sym{***}$ & $-1.113\sym{***}$ \\
                    & $(0.216)$         & $(0.262)$         \\
\addlinespace
Price               & $0.106\sym{***}$  & $0.094\sym{**}$   \\
                    & $(0.036)$         & $(0.041)$         \\
\addlinespace
Block$\times$Price  & $-0.008$          & $0.006$           \\
                    & $(0.022)$           & $(0.023)$         \\
\addlinespace
Constant            & $1.378\sym{***}$  & $1.385\sym{***}$  \\
                    & $(0.199)$         & $(0.226)$         \\
\midrule
Individual fixed effects  & Yes         & Yes               \\
Product fixed effects     & Yes         & Yes               \\
\midrule
Observations        & $5,100$          & $5,100$         \\      
Left-censored       & -                & $619$           \\
Right-censored      & -                & $87$            \\
Number of subjects  & $85$             & $85$ \\
\bottomrule
\end{tabular}
}


==> Attribute/Tables/Regression_LinearTobit.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
%\begin{tabular}{l*{4}{D{.}{.}{-1}}}
\begin{tabular}{lcccc}
\toprule
                    & Linear           & Linear           & Tobit            & Tobit \\
                    & (1)              & (2)              & (3)              & (4)               \\
\midrule
Block               & $-0.988\sym{***}$& $-0.988\sym{***}$& $-1.149\sym{***}$& $-1.144\sym{***}$ \\
                    & $(0.231)$        & $(0.232)$        & $(0.268)$        & $(0.268)$         \\
\addlinespace
Price               & $0.290\sym{***}$ & -                & $0.295\sym{***}$ & -                 \\
                    & $(0.029)$        & -                & $(0.029)$        & -                 \\
\addlinespace
Block$\times$Price  & $-0.003$         & $-0.003$         & $0.008$          & $0.008$           \\
                    & $(0.024)$        & $(0.024)$        & $(0.024)$        & $(0.024)$         \\
\addlinespace
Constant            & $1.155\sym{***}$ & $2.254\sym{***}$ &$1.109\sym{***}$  & $2.207\sym{***}$  \\
                    & $(0.151)$        & $(0.198)$        & $(0.156)$        & $(0.204)$         \\
\midrule
Individual fixed effects & Yes         &  Yes             & Yes              & Yes  \\
Product fixed effects    & No          &  Yes             & No               & Yes  \\
\midrule     
Observations        & $4,798$          & $4,798$          & $4,798$          & $4,798$  \\
Left-censored       & -                &-                 & $317$            & $317$ \\
Right-censored      & -                &-                 & $87$             & $87$ \\
Number of subjects  & $85$             & $85$             & $85$             & $85$  \\
\bottomrule
\end{tabular}
}


==> Attribute/Tables/Regression_OLS.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{lccc}
\toprule
                &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         \\
\midrule
Block           &   $-0.997\sym{***}$&   $-0.997\sym{***}$&   $-0.988\sym{***}$\\
                &  (0.224)         &  (0.224)         &  (0.230)         \\
\addlinespace
Price           & $\cdot$          &    0.116\sym{***}&    0.118\sym{***}\\
                &                  &  (0.030)         &  (0.035)         \\
\addlinespace
Block$\times$Price      & $\cdot$          & $\cdot$          &   $-0.003$         \\
                &                  &                  &  (0.024)         \\
\addlinespace
Constant        &    2.931\sym{***}&    2.445\sym{***}&    2.440\sym{***}\\
                &  (0.112)         &  (0.196)         &  (0.200)         \\
\midrule

Product Effects &       No         &      Yes         &      Yes         \\
Fixed Effects   &      Yes         &      Yes         &      Yes         \\
\midrule
Observations    &     4798         &     4798         &     4798         \\
\bottomrule
\hline
\end{tabular}
}


==> Attribute/Tables/Regression_four.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
%\begin{tabular}{l*{4}{D{.}{.}{-1}}}
\begin{tabular}{lcccc}
\toprule
                    &\multicolumn{2}{c}{Linear}              &\multicolumn{2}{c}{Tobit}  \\
                    \cmidrule(lr){2-3}\cmidrule(lr){4-5}
                    &\multicolumn{1}{c}{(1)}         &\multicolumn{1}{c}{(2)}         &\multicolumn{1}{c}{(3)}         &\multicolumn{1}{c}{(4)}\\
\midrule
Block               & $-0.997\sym{***}$& $-0.988\sym{***}$& $-1.141\sym{***}$& $-1.144\sym{***}$ \\
                    & $(0.224)$        &  $(0.232)$       & $(0.261)$        & $(0.268)$         \\
\addlinespace
Block$\times$Price  & -                & $-0.003$         & -                & $0.008$           \\
                    & -                & $0.024$          & -                & $(0.024)$         \\
\addlinespace
Constant            & $2.931\sym{***}$ & $2.254\sym{***}$ & $2.936\sym{***}$ & $2.207\sym{***}$  \\
                    & $(0.187)$        & $(0.198)$        & $(0.198)$        & $(0.204)$         \\
\midrule
Individual fixed effects  &  No              & Yes              & No               & Yes               \\
Product fixed effects     &  No              & Yes              & No               & Yes               \\
\midrule      
Observations        & $4,798$          & $4,798$          & $4,798$          & $4,798$ \\
Left-censored       & -                & -                & $317$            & $317$ \\
Right-censored      & -                & -                & $87$             & $87$ \\
\bottomrule
\end{tabular}
}


==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}
